Towards Generalizable Diabetic Retinopathy Grading in Unseen Domains

Diabetic Retinopathy (DR) is a common complication of diabetes and a leading cause of blindness worldwide. Early and accurate grading of its severity is crucial for disease management. Although deep learning has shown great potential for automated DR grading, its real-world deployment is still challenging due to distribution shifts among source and target domains, known as the domain generalization problem. Existing works have mainly attributed the performance degradation to limited domain shifts caused by simple visual discrepancies, which cannot handle complex real-world scenarios. Instead, we present preliminary evidence suggesting the existence of three-fold generalization issues: visual and degradation style shifts, diagnostic pattern diversity, and data imbalance. To tackle these issues, we propose a novel unified framework named Generalizable Diabetic Retinopathy Grading Network (GDRNet). GDRNet consists of three vital components: fundus visual-artifact augmentation (FundusAug), dynamic hybrid-supervised loss (DahLoss), and domain-class-aware re-balancing (DCR). FundusAug generates realistic augmented images via visual transformation and image degradation, while DahLoss jointly leverages pixel-level consistency and image-level semantics to capture the diverse diagnostic patterns and build generalizable feature representations. Moreover, DCR mitigates the data imbalance from a domain-class view and avoids undesired over-emphasis on rare domain-class pairs. Finally, we design a publicly available benchmark for fair evaluations. Extensive comparison experiments against advanced methods and exhaustive ablation studies demonstrate the effectiveness and generalization ability of GDRNet.

==> subb.tex <==
\section{Appendix}

\begin{figure}
    \vspace{-4mm}
    \centering
    \includegraphics[width=1\textwidth]{figures/supp_domain.pdf}
    \caption{\small{The RGB statistics, category histograms and proliferative DR (PDR) samples from other five datasets/domains.}}
    \label{fig:supp_domain}
    \vspace{-4mm}
\end{figure}

\begin{figure}
    \vspace{-4mm}
    \centering
    \includegraphics[width=1.0\textwidth]{figures/operations.pdf}
    \caption{\small{Augmentation pipelines and parameter ranges of all FundusAug.}}
    \label{fig:operations}
    \vspace{-4mm}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{figures/augmentedviews.pdf}
    \caption{\small{Augmented samples via FundusAug. These views show the effectiveness of FundusAug in increasing the training sample diversity.}}
    \label{fig:augmentedviews}
    \vspace{-4mm}
\end{figure}

\begin{table*}
    \renewcommand\arraystretch{1.1}
    \centering
    \caption{\small{Controllable parameters during training.}}
    \label{tab:fundusparameters}   
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
    Parameters & Epochs &Learning rate (decayed) & Batch size & Weight decay & Momentum value & Intensity $\beta$ & Temperature $\tau$ \\
    \hline
    \hline
    Comparison methods &100 &$10^{-3}$ ($10^{-4}$) &$16$ &$5\times10^{-4}$ &$0.9$ &\textbf{-} &\textbf{-} \\
    GDRNet (DG)  &100 &$10^{-3}$ ($10^{-4}$) &$16$ &$5\times10^{-4}$ &$0.9$ &$0.5$ &$0.1$ \\
    GDRNet (ESDG) &100 &$10^{-3}$ ($10^{-4}$) &$16$ &$5\times10^{-4}$ &$0.9$ &$0.5$ &$0.01$ \\
  
    \bottomrule
    \end{tabular}
    }
    \vspace{-4mm}
\end{table*}


\begin{table*}
    \renewcommand\arraystretch{1.1}
    \centering
    \caption{\small{A brief summary for comparison methods.}}
    \label{tab:comparisonsfundus}   
    \resizebox{1.0\textwidth}{!}{%
    \begin{tabular}{c|c|l}
    \toprule
    \multicolumn{1}{c|}{Name} &  \multicolumn{1}{c|}{Category} & \multicolumn{1}{c}{Brief Description} \\
        
    \hline
    GREEN & OSD & \multicolumn{1}{m{12cm}}{Utilize class dependency priors for DR grading via a graph convolutional network.} \\
    \hline
    CABNet & OSD &  \multicolumn{1}{m{12cm}}{Learn discriminative features for each grade via the categorical attention block.} \\
    \hline
    Mixup & DGT &  \multicolumn{1}{m{12cm}}{Mix both images and labels to improve generalization ability.} \\
    \hline
    MixStyle & DGT &  \multicolumn{1}{m{12cm}}{Mix feature statistics of training samples across domains to improve generalization.} \\    
    \hline
    DDAIG & DGT &  \multicolumn{1}{m{12cm}}{Generate novel perturbed images to improve generalization via adversarial training.} \\    
    \hline
    ATS & DGT &  \multicolumn{1}{m{12cm}}{Advances Teacher-Student learning in an adversarial learning manner.} \\    
    \hline
    DRGen & DGT &  \multicolumn{1}{m{12cm}}{Combine Fishr and SWAD, which aims to find the flat optima.} \\    
    \hline
    Fishr & FRL &  \multicolumn{1}{m{12cm}}{Enforce domain invariance in the space of the gradients of the loss.} \\    
    \hline
    MDLT & FRL &  \multicolumn{1}{m{12cm}}{Based on the prototype learning, address data imbalance and domain shifts.} \\    
    \bottomrule
    \end{tabular}
    }
    \vspace{-4mm}
\end{table*}

% Method Description
% Emphasize they have the same learning parameters and settings with GDRNet.
% List the augmentation.

% In this section, we will briefly introduce comparison methods used in the main content to show the fairness of our experiments.
% Spefically, we compare our GDRNet with three sets of methods, i.e., ophthalmic disease diagnosis, domain generalization techniques, and feature representation learning.
% The reason for such design of experiments is that we aim to tackle a generalizable ophthalmic diasese grading in unseen domains by learning generalizable feature representation.
% Thus, the experimental design can illustrate our critical contributions aming to tackle DGDR.

% \textbf{Ophthalmic disease diagnosis.} 
% GREEN \cite{liu2020green} utilizes a class dependency prior for DR grading tasks based on a graph convolutional network.
% CABNet \cite{he2020cabnet} learns discriminative features for each severity level via the categorical attention block, aiming to address robust DR grading.

% \textbf{Domain generalization techniques.} 
% Mixup \cite{zhangmixup} is a classic augmentation method in which images are mixed to improve robustness.
% Mixstyle \cite{zhoudomain} conducts a mixing of feature statistics of training samples across domains to improve the robustness of models.
% DDAIG \cite{zhou2020deep} adopts adversarial training to generate beneficial perturbed images to achieve improvement of generalization ability.
% Similar to DDAIG, ATS \cite{yang2021adversarial} adopts adversarial training to generate beneficial perturbed images by maximizing 

% \textbf{Feature representation learning.}
% Fishr \cite{rame2022fishr} is xxxxx
% MDLT \cite{yang2022multi} is xxxxx


% \subsubsection{Ablation Details and Visualization}

% Due to the paragraph limitation, we only report AUC scores of the ablation study. 
% To give readers a more clear understanding of impacts from three components and sense of varying severity of three-fold generalization issues in different domains, we report all metrics in the table \ref{tab:comparisonsfundus}.
% The results still illustrates the effectiveness of GDRNet facing varying generalization situation and DGDR is non-trivial.
% Further, we conduct a visualization analysis for features learned by the vanilla model with CE (ERM) and GDRNet, as shown in Fig. \ref{fig:visualization}.
% Both models are trained on five domains including DeepDR\cite{wang2021deep}, Messidor\cite{abramoff2016improved}, IDRID\cite{porwal2018indian}, FGADR\cite{FGADR}, and RLDR\cite{icpr2020-LesionNet}, and APTOS\cite{APTOS} is the test domain.
% As expected, GDRNet can learn features with sufficient intra-class variations while ERM trained by CE learns dense feature, leading to increase of intra-domain performance but decrease of unseen-domain performance.
% Notably, GDR not only improve the performance towards unseen domains but also maintain intra-domain performance non-decreased, showing its effectiveness and generalization ability.

\begin{table*}
        \renewcommand\arraystretch{1.2}
        \centering
        \caption{\small{Ablation studies on proposed components under the DG test.}}
        \label{tab:comparisonsfundus}
        \resizebox{1.0\textwidth}{!}{%
        \scalebox{0.69}{
        \begin{tabular}{c|ccc|ccc|ccc|ccc|ccc|ccc|ccc}
        \toprule
             Target &\multicolumn{3}{c|}{APTOS} &\multicolumn{3}{c|}{DeepDR}  &\multicolumn{3}{c|}{FGADR}&\multicolumn{3}{c|}{IDRID} &\multicolumn{3}{c|}{Messidor}  &\multicolumn{3}{c|}{RLDR} &\multicolumn{3}{c}{Average}\\
            \hline
            Metrics & AUC &ACC & F1 & AUC &ACC & F1&  AUC &ACC & F1 & AUC &ACC & F1 & AUC &ACC & F1&  AUC &ACC & F1 &  AUC &ACC & F1\\
            \hline
            \hline
            ERM &75.0 &44.4 &38.9 &77.0 &39.5 &34.3 &66.2 &32.0 &27.1 &82.3 &50.0 &44.1 &79.1 &60.7 &43.5 &75.9 &36.5 &35.7 &75.9 &43.8 &37.3\\
            \midrule
            Model A &77.2 &53.8 &40.6 &80.2 &42.0 &37.7 &74.9 &42.7 &37.7 &82.8 &53.1 &45.3 &80.5 &61.1 &47.3 &80.2 &43.6 &40.0 &79.3 &49.4 &41.4\\
            Model B &75.4 &38.6 &32.7 &79.1 &41.4 &34.3 &68.4 &33.0 &27.5 &82.7 &50.2 &45.1 &77.9 &62.6 &45.8 &78.9 &41.8 &39.9 &77.1 &44.6 &37.5\\
            Model C &75.6 &47.0 &40.2 &78.8 &46.2 &38.3 &67.3 &33.1 &26.6 &82.6 &52.1 &45.7 &78.9 &59.5 &47.4 &78.4 &40.4 &37.3 &76.9 &46.4 &39.2\\
            Model D &77.7 &54.9 &42.0 &81.2 &47.5 &40.0 &75.3 &45.3 &36.5 &82.0 &53.1 &44.4 &79.1 &62.2 &42.0 &80.6 &44.1 &40.9 &79.3 &51.2 &41.0\\
            \midrule
            Model E &77.3 &59.6 &42.4 &83.4 &52.0 &42.7 &77.4 &40.7 &31.1 &83.6 &53.5 &43.8 &80.2 &68.9 &42.9 &80.8 &43.8 &39.1 &80.5 &53.1 &40.3\\
            Model F &77.4 &51.4 &40.6 &83.9 &54.7 &46.6 &77.9 &47.9 &42.4 &83.4 &52.3 &44.5 &82.4 &65.2 &50.8 &83.3 &49.0 &45.0 &81.4 &53.4 &45.0\\
            Model G &80.4 &68.7 &45.4 &85.1 &56.4 &43.5 &78.7 &45.0 &35.3 &83.7 &49.4 &39.1 &84.9 &67.6 &50.6 &82.0 &46.7 &42.5 &82.5 &55.6 &42.7\\
            \midrule
            \textbf{GDRNet} &79.9 &66.8 &46.0 &84.7 &53.1 &45.3 &80.8 &45.3 &39.4 &84.0 &40.3 &35.9 &83.2 &63.4 &50.9 &82.9 &45.8 &43.5 &82.6 &52.5 &43.5\\
            \bottomrule
            \end{tabular}
    }}
    \label{tab:SDG}
    \vspace{-4mm}
\end{table*}
